CCTVBench: Contrastive Consistency Traffic VideoQA Benchmark for Multimodal LLMs

Safety-critical traffic reasoning requires contrastive consistency: models must detect true hazards when an accident occurs, and reliably reject plausible-but-false hypotheses under near-identical counterfactual scenes. We present CCTVBench, a Contrastive Consistency Traffic VideoQA Benchmark built on paired real accident videos and world-model-generated counterfactual counterparts, together with minimally different, mutually exclusive hypothesis questions. CCTVBench enforces a single structured decision pattern over each video question quadruple and provides actionable diagnostics that decompose failures into positive omission, positive swap, negative hallucination, and mutual-exclusivity violation, while separating video versus question consistency. Experiments across open-source and proprietary video LLMs reveal a large and persistent gap between standard per-instance QA metrics and quadruple-level contrastive consistency, with unreliable none-of-the-above rejection as a key bottleneck. Finally, we introduce C-TCD, a contrastive decoding approach leveraging a semantically exclusive counterpart video as the contrast input at inference time, improving both instance-level QA and contrastive consistency.

==> table/2.videopair_behavior.tex <==
\begin{table}[t]
\centering
\small
\caption{Hallucination and omission rates under positive and negative queries. All values are percentages.}

\setlength{\tabcolsep}{6pt}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{l c c c c}
\toprule
\multirow{2}{*}{\textbf{Model}} &
\multirow{2}{*}{\textbf{Size}} &
\multicolumn{3}{c}{\textbf{Hallucination and Omission Table (\%)}} \\
\cmidrule(lr){3-5}
 &  & Hall@$q+\downarrow$ & Omiss@$q+\downarrow$ & Hall@$q-\downarrow$ \\
\midrule
\multicolumn{5}{c}{\textit{Open-source Models}} \\
\midrule
% InternVL3.5            & 1B  & 33.99 & 57.57 & 28.64 \\
InternVL3.5            & 2B  & 39.67 & 50.20 & 26.62 \\
% InternVL3.5            & 4B  & 22.62 & 62.86 &  8.72 \\
InternVL3.5            & 8B  & 44.01 & 38.44 & 21.67 \\
PLLaVA                 & 13B & 39.28 & 50.25 & 21.55 \\
PLLaVA                 & 7B  & 25.21 & 67.19 & 11.20 \\
% Qwen2.5-VL             & 7B  & 24.87 & 62.07 &  \textbf{4.95} \\
Qwen3-VL               & 2B  & 45.13 & 40.52 & 23.07 \\
% Qwen3-VL-Thinking      & 2B  & 30.61 & 58.19 & 20.99 \\
% Qwen3-VL               & 4B  & 19.92 & 61.23 &  5.51 \\
Qwen3-VL               & 8B  & \cellcolor{black!15}{\textbf{20.77}} & \cellcolor{black!15}{68.82} & \cellcolor{black!15}{\textbf{4.28}} \\

% Video-R1               & 7B  & 24.42 & 63.14 &  4.95 \\
VideoChatGPT           & 7B  & 64.55 & 38.10 & 62.35 \\
VideoLLaMA3            & 2B  & 54.31 & 39.17 & 46.26 \\
VideoLLaMA3            & 7B  & 61.45 & 32.64 & 43.95 \\
Phi-4-Multimodal       & 14B & 62.13 & \textbf{30.67} & 49.69 \\
\midrule
\multicolumn{5}{c}{\textit{Proprietary Models}} \\
\midrule
Gemini-2.5             & flash-lite  & 44.18 & 38.10 &  9.12 \\
Gemini-2.5             & flash       & 46.88 & \textbf{37.99} & 10.13 \\
GPT-5                  & nano        & \textbf{27.86} & 72.43 &  \textbf{5.18} \\
GPT-5                  & mini        & 38.55 & 40.63 &  7.71 \\
\bottomrule
\end{tabular}}
\label{tab:qplus_taxonomy}
\end{table}
